Graph Treewidth and Geometric Thickness Parameters

Consider a drawing of a graph $G$ in the plane such that crossing edges are coloured differently. The minimum number of colours, taken over all drawings of $G$, is the classical graph parameter "thickness". By restricting the edges to be straight, we obtain the "geometric thickness". By further restricting the vertices to be in convex position, we obtain the "book thickness". This paper studies the relationship between these parameters and treewidth. Our first main result states that for graphs of treewidth $k$, the maximum thickness and the maximum geometric thickness both equal $\lceil{k/2}\rceil$. This says that the lower bound for thickness can be matched by an upper bound, even in the more restrictive geometric setting. Our second main result states that for graphs of treewidth $k$, the maximum book thickness equals $k$ if $k \leq 2$ and equals $k+1$ if $k \geq 3$. This refutes a conjecture of Ganley and Heath [Discrete Appl. Math. 109(3):215-221, 2001]. Analogous results are proved for outerthickness, arboricity, and star-arboricity.

==> myCommands.tex <==
\DeclareFontShape{OT1}{cmr}{b}{sc}
{<5><6><7><8><9><10><12><10.95><14.4><17.28><20.74><24.88>cmbcsc10}{}
\DeclareFontShape{OT1}{cmr}{bx}{sc}
{<5><6><7><8><9><10><12><10.95><14.4><17.28><20.74><24.88>cmbcsc10}{}

\DeclareFontShape{OT1}{cmr}{b}{tt}
{<5><6><7><8><9><10><12><10.95><14.4><17.28><20.74><24.88>cmbtt10}{}
\DeclareFontShape{OT1}{cmr}{bx}{tt}
{<5><6><7><8><9><10><12><10.95><14.4><17.28><20.74><24.88>cmbtt10}{}

%%%%%%%%%%%%%%%%

\newcommand{\NP}{\ensuremath{\mathcal{NP}}}

\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}

\newcommand{\aaa}{\textup{(a)}}
\newcommand{\bbb}{\textup{(b)}}
\newcommand{\ccc}{\textup{(c)}}
\newcommand{\ddd}{\textup{(d)}}
\newcommand{\eee}{\textup{(e)}}

\newcommand{\myKeywords}[1]{\medskip\noindent \hspace*{8mm}
\begin{minipage}[t]{\textwidth-16mm} \textbf{Keywords}: \small #1
\end{minipage}}

\newcommand{\FancyFootnotes}{\renewcommand{\thefootnote}{\fnsymbol{footnote}}}
\newcommand{\FancyFootnotesOff}{\renewcommand{\thefootnote}{\arabic{footnote}}}

\newcommand{\YES}{\textup{\textsf{YES}}}
\newcommand{\NO}{\textup{\textsf{NO}}}

\newcommand{\Prob}[1]{\ensuremath{\textbf{\textup{P}}#1}}
\newcommand{\PROB}[1]{\ensuremath{\textbf{P}\left[#1\right]}}

\newcommand{\e}{\ensuremath{\boldsymbol{e}}}

\newcommand{\Case}[3]{\medskip\boldmath\textbf{Case #1 --- #2}\unboldmath#3: }
\newcommand{\case}[2]{\boldmath\textbf{Case #1. #2:}\unboldmath}
\newcommand{\BoldSimpleCase}[2]{\boldmath\textbf{Case #1. #2:}\unboldmath}

\newcommand{\raised}[1]{\footnotesize\raisebox{1ex}{#1}\normalsize}
\newcommand{\lowered}[1]{\footnotesize\raisebox{-1ex}{#1}\normalsize}

\newcommand{\paran}[1]{\textup{(}#1\textup{)}}

\newcommand{\Succ}[2][]{\ensuremath{\protect\textup{succ}_{#1}(#2)}}
\newcommand{\Pred}[2][]{\ensuremath{\protect\textup{pred}_{#1}(#2)}}
\newcommand{\set}[1]{\ensuremath{\protect\{#1\}}}
\newcommand{\SET}[1]{\ensuremath{\protect\left\{#1\right\}}}
\newcommand{\maxm}[1]{\ensuremath{\protect\max\set{#1}}}
\newcommand{\MAXM}[1]{\ensuremath{\protect\max\SET{#1}}}
\newcommand{\minm}[1]{\ensuremath{\protect\min\set{#1}}}
\newcommand{\MINM}[1]{\ensuremath{\protect\min\SET{#1}}}
\newcommand{\bracket}[1]{\ensuremath{\protect\left(#1\right)}}
\newcommand{\BRACKET}[1]{\ensuremath{\protect\left(#1\right)}}
\newcommand{\BFRAC}[2]{\ensuremath{\protect\left(\frac{#1}{#2}\right)}}
\newcommand{\bb}[1]{\ensuremath{\protect\Big(#1\Big)}}
\newcommand{\ANGLE}[1]{\ensuremath{\protect\langle#1\rangle}}
\newcommand{\ABS}[1]{\ensuremath{\protect\left|#1\right|}}
\newcommand{\CARD}[1]{\ensuremath{\protect\left|#1\right|}}
\newcommand{\abs}[1]{\ensuremath{\protect|#1|}}
\newcommand{\card}[1]{\ensuremath{\protect|#1|}}
\newcommand{\ceil}[1]{\ensuremath{\protect\lceil#1\rceil}}
\newcommand{\CEIL}[1]{\ensuremath{\protect\left\lceil#1\right\rceil}}
\newcommand{\FLOOR}[1]{\ensuremath{\protect\left\lfloor#1\right\rfloor}}
\newcommand{\floor}[1]{\ensuremath{\protect\lfloor#1\rfloor}}

\newcommand{\eqdef}[0]{\ensuremath{\substack{\text{ \emph{def} }\\=}}}
\newcommand{\HALF}{\ensuremath{\protect\dfrac{1}{2}}}
\newcommand{\half}{\ensuremath{\protect\tfrac{1}{2}}}
\newcommand{\THREEHALVES}{\ensuremath{\protect\dfrac{3}{2}}}
\newcommand{\threehalves}{\ensuremath{\protect\tfrac{3}{2}}}
\newcommand{\fivehalves}{\ensuremath{\protect\tfrac{5}{2}}}
\newcommand{\fourthirds}{\ensuremath{\protect\tfrac{4}{3}}}
\newcommand{\FOURTHIRDS}{\ensuremath{\protect\dfrac{4}{3}}}
\newcommand{\FIVEHALVES}{\ensuremath{\protect\dfrac{5}{2}}}
\newcommand{\eighth}{\ensuremath{\protect\tfrac{1}{8}}}
\newcommand{\EIGHTH}{\ensuremath{\protect\dfrac{1}{8}}}
\newcommand{\threeeighths}{\ensuremath{\protect\tfrac{3}{8}}}
\newcommand{\THREEEIGHTHS}{\ensuremath{\protect\dfrac{3}{8}}}
\newcommand{\QUARTER}{\ensuremath{\protect\dfrac{1}{4}}}
\newcommand{\quarter}{\ensuremath{\protect\tfrac{1}{4}}}
\newcommand{\SIXTH}{\ensuremath{\protect\dfrac{1}{6}}}
\newcommand{\sixth}{\ensuremath{\protect\tfrac{1}{6}}}
\newcommand{\THIRD}{\ensuremath{\protect\dfrac{1}{3}}}
\newcommand{\third}{\ensuremath{\protect\tfrac{1}{3}}}
\newcommand{\THREEQUARTS}{\ensuremath{\protect\dfrac{3}{4}}}
\newcommand{\threequarts}{\ensuremath{\protect\tfrac{3}{4}}}
\newcommand{\TWOTHIRDS}{\ensuremath{\protect\dfrac{2}{3}}}
\newcommand{\twothirds}{\ensuremath{\protect\tfrac{2}{3}}}

%\newcommand{\outdeg}[1]{\mbox{(out)deg}\bracket{#1}}
%\newcommand{\outdeg}[2][]{\ensuremath{\protect\textup{deg}_{#1}(#2)}} %^+
%\newcommand{\indeg}[2][]{\ensuremath{\protect\textup{deg}^-_{#1}(#2)}}
\newcommand{\maxoutdeg}[1]{\ensuremath{\protect\Delta^+(#1)}}
\newcommand{\maxindeg}[1]{\ensuremath{\protect\Delta^-(#1)}}

\newcommand{\ontop}[2]{\protect\substack{#1\\#2}}
\newcommand{\ontoptop}[3]{\protect\substack{#1\\#2\\#3}}
\newcommand{\range}[3]{\protect\left\{#1,#2,\ldots,#3\right\}}

\newcommand{\etal}{~\emph{et~al.}~}

\newcommand{\arc}[1]{\ensuremath{\protect\overrightarrow{#1}}}
\newcommand{\ArcGraph}[1]{\overleftrightarrow{#1}}

\newcommand{\YDelta}{\protect{Y}\Delta}
\newcommand{\DeltaY}{\protect\Delta{Y}}

\newcommand{\leftbrace}[1]{\left\{#1\right.}
\newcommand{\rightbrace}[1]{\left.#1\right\}}

\newcommand{\lb}[1]{\ensuremath{\protect\Omega(#1)}}
\newcommand{\tb}[1]{\ensuremath{\protect\Theta(#1)}}
\newcommand{\ub}[1]{\ensuremath{\protect\mathcal{O}(#1)}}

%\newcommand{\LB}[1]{\ensuremath{\protect\Omega\!\left(#1\right)}}
%\newcommand{\TB}[1]{\ensuremath{\protect\Theta\!\left(#1\right)}}
%\newcommand{\UB}[1]{\ensuremath{\protect\mathcal{O}\!\left(#1\right)}}

\newcommand{\oh}[1]{\ensuremath{\protect o\!\left(#1\right)}}
\newcommand{\Oh}[1]{\ensuremath{\protect\mathcal{O}(#1)}}
\newcommand{\bigOh}[1]{\ensuremath{\protect\mathcal{O}\!\big(#1\big)}}
\newcommand{\BigOh}[1]{\ensuremath{\protect\mathcal{O}\!\Big(#1\Big)}}
\newcommand{\OH}[1]{\ensuremath{\protect\mathcal{O}\!\left(#1\right)}}

\newcommand{\plane}[1]{\mbox{\ensuremath{(#1)}-plane}}


\newcommand{\EndProof}[1]{
\begin{minipage}[b]{\textwidth-1cm}
#1
\end{minipage}\hfill\qed
\vspace*{1ex}
\renewcommand{\qed}{}
}

\newcommand{\contradiction}
{\raisebox{0.7ex}{
\hspace*{1mm}
\pspicture(0,0)
\psset{unit=4mm}
\SpecialCoor
\pscircle(0;0){1}
\pscircle*(0.5;45){0.15}
\pscircle*(0.5;135){0.15}
\psarc(0.5;270){0.3}{10}{170}
\endpspicture}
\hspace*{0mm}}

\newcommand{\Figure}[4][htb]{
\begin{figure}[#1]
	\vspace*{1ex}
	\begin{center}#3\end{center}
	\vspace*{-1ex}
	\caption{\figlabel{#2}#4}
\end{figure}
}

\newcommand{\OneColumnFigure}[4][tb]{
\begin{figure*}[#1]
	\vspace*{1ex}
	\begin{center}#3\end{center}
	\vspace*{-3ex}
	\caption{\figlabel{#2}#4}
\end{figure*}
}

\newcommand{\spacing}[1]{
\renewcommand{\baselinestretch}{#1}
\setlength{\footnotesep}{\baselinestretch\footnotesep}}

\newcommand{\Settings}[5]{
% 1: Spacing 
% 2: LRMargin
% 3: TBMargin
% 4: Head Sep
% 5: foot skip

% controls line spacing
\renewcommand{\baselinestretch}{#1}
\setlength{\footnotesep}{\baselinestretch\footnotesep}

% the size of margin notes
\setlength{\marginparwidth}{0mm}
\setlength{\marginparsep}{0mm}
\setlength{\marginparpush}{0mm}

%  These define the size of actual margins around the text
\newlength{\LRmargin}
\setlength{\LRmargin}{#2}
\newlength{\TBmargin}
\setlength{\TBmargin}{#3}

%  Now adjust page length parameters to reflect desired margins
\setlength{\voffset}{-1in}           % cancels default printer margin
\setlength{\hoffset}{-1in}           % cancels default printer margin

\setlength{\headsep}{#4}
\setlength{\footskip}{#5}

\setlength{\oddsidemargin}{\LRmargin}
\setlength{\evensidemargin}{\LRmargin}
\setlength{\topmargin}{\TBmargin}

\setlength{\textheight}{\paperheight}
\addtolength{\textheight}{-1in}			% default printer margin
\addtolength{\textheight}{-1.0\voffset}
\addtolength{\textheight}{-2.0\TBmargin}	% top and bottom
\addtolength{\textheight}{-1.0\headheight}
\addtolength{\textheight}{-1.0\headsep}
\addtolength{\textheight}{-1.0\footskip}

\setlength{\textwidth}{\paperwidth}
\addtolength{\textwidth}{-1.0in}		% default printer margin
\addtolength{\textwidth}{-1.0\hoffset}
\addtolength{\textwidth}{-2.0\LRmargin}		% left and right margin
}

\newcommand{\NewSettings}[6]{
% 1: Spacing 
% 2: LeftMargin
% 3: RightMargin
% 4: TBMargin
% 5: Head Sep
% 6: foot skip

% contols line spacing
\renewcommand{\baselinestretch}{#1}
\setlength{\footnotesep}{\baselinestretch\footnotesep}

% the size of margin notes
\setlength{\marginparwidth}{0mm}
\setlength{\marginparsep}{0mm}
\setlength{\marginparpush}{0mm}

%  These define the size of actual margins around the text
\newlength{\Lmargin}
\setlength{\Lmargin}{#2}
\newlength{\Rmargin}
\setlength{\Rmargin}{#3}
\newlength{\TBmargin}
\setlength{\TBmargin}{#4}

%  Now adjust page length parameters to reflect desired margins
\setlength{\voffset}{-1in}           % cancels default printer margin
\setlength{\hoffset}{-1in}           % cancels default printer margin

\setlength{\headsep}{#5}
\setlength{\footskip}{#6}

\setlength{\oddsidemargin}{\Lmargin}
\setlength{\evensidemargin}{\Lmargin}
\setlength{\topmargin}{\TBmargin}

\setlength{\textheight}{\paperheight}
\addtolength{\textheight}{-1in}			% default printer margin
\addtolength{\textheight}{-1.0\voffset}
\addtolength{\textheight}{-2.0\TBmargin}	% top and bottom
\addtolength{\textheight}{-1.0\headheight}
\addtolength{\textheight}{-1.0\headsep}
\addtolength{\textheight}{-1.0\footskip}

\setlength{\textwidth}{\paperwidth}
\addtolength{\textwidth}{-1.0in}		% default printer margin
\addtolength{\textwidth}{-1.0\hoffset}
\addtolength{\textwidth}{-1.0\Lmargin}		% left and right margin
\addtolength{\textwidth}{-1.0\Rmargin}		% left and right margin
}

\newcommand{\FullSettings}[7]{
% 1: Spacing 
% 2: LeftMargin
% 3: RightMargin
% 4: TopMargin
% 5: BottomMargin
% 6: Head Sep
% 7: foot skip

% contols line spacing
\renewcommand{\baselinestretch}{#1}
\setlength{\footnotesep}{\baselinestretch\footnotesep}

% the size of margin notes
\setlength{\marginparwidth}{0mm}
\setlength{\marginparsep}{0mm}
\setlength{\marginparpush}{0mm}

%  These define the size of actual margins around the text
\newlength{\Lmargin}
\setlength{\Lmargin}{#2}
\newlength{\Rmargin}
\setlength{\Rmargin}{#3}
\newlength{\Tmargin}
\setlength{\Tmargin}{#4}
\newlength{\Bmargin}
\setlength{\Bmargin}{#5}

%  Now adjust page length parameters to reflect desired margins
\setlength{\voffset}{-1in}           % cancels default printer margin
\setlength{\hoffset}{-1in}           % cancels default printer margin

\setlength{\headsep}{#6}
\setlength{\footskip}{#7}

\setlength{\oddsidemargin}{\Lmargin}
\setlength{\evensidemargin}{\Lmargin}
\setlength{\topmargin}{\Tmargin}

\setlength{\textheight}{\paperheight}
\addtolength{\textheight}{-1in}			% default printer margin
\addtolength{\textheight}{-1.0\voffset}
\addtolength{\textheight}{-1.0\Tmargin}
\addtolength{\textheight}{-1.0\Bmargin}
\addtolength{\textheight}{-1.0\headheight}
\addtolength{\textheight}{-1.0\headsep}
\addtolength{\textheight}{-1.0\footskip}

\setlength{\textwidth}{\paperwidth}
\addtolength{\textwidth}{-1.0in}		% default printer margin
\addtolength{\textwidth}{-1.0\hoffset}
\addtolength{\textwidth}{-1.0\Lmargin}
\addtolength{\textwidth}{-1.0\Rmargin}
}

\newlength{\marginboxwidth}

\newcommand{\OldComment}[1]{
\setlength{\marginboxwidth}{\evensidemargin}
\addtolength{\marginboxwidth}{-2em}
\marginpar{\hspace*{1em}\fbox{\parbox{\marginboxwidth}{\setlength{\baselineskip}{3ex}#1}}}}

\usepackage{pifont}


\newcommand{\vc}[1]
{
{\textcolor{red}{\ding{43}}}
\marginpar{\vspace*{-3mm}{\textcolor{red}{{\ding{42}}}}\fbox{\begin{minipage}
{24mm}\setlength{\baselineskip}{0ex}
{{\scriptsize #1}}\end{minipage}}
}}



\newcommand{\Comment}[1]
{
\ding{43}
\setlength{\marginboxwidth}{\paperwidth}
\addtolength{\marginboxwidth}{-1.0\textwidth}
\addtolength{\marginboxwidth}{-1.0\evensidemargin}	% Lmargin
\addtolength{\marginboxwidth}{-30mm}
\marginpar{\hspace*{1em}\fbox{\parbox{\marginboxwidth}{\setlength{\baselinesOBkip}{3ex}#1}}}
}

\newcommand{\NewComment}[2][2cm]
{
\marginpar{\hspace*{1em}\fbox{\parbox{#1}{\setlength{\baselineskip}{3ex}#2}}}
}

\newcommand{\COMMENT}[1]{\medskip\noindent\framebox{\parbox{\textwidth-2mm}{#1}}\medskip}

\newcommand{\comment}[1]{~\newline\medskip\noindent\framebox{\parbox{\textwidth-2mm}{#1}}\medskip}

\renewcommand{\comment}[1]{
\medskip\noindent
\framebox{\parbox{\textwidth-2mm}{#1}}
\medskip}

%%%%%%%%%%%%%% vida %%%%%%%%%%%%%%%%
\newcommand{\Change}[1]
{
\marginpar{~\\~\hspace*{4.5em}\framebox[0cm]{\parbox{0cm}{\setlength{\baselineskip}{0ex}~\vspace{#1}}}}
}

\newcommand{\CommentVida}[1]
{
{\textcolor{red}*}
\marginpar{{\textcolor{red}{$\Longrightarrow$}}\fbox{\begin{minipage}{26.7mm}\setlength{\baselineskip}{0ex}
{{\scriptsize #1}}\end{minipage}}
}}


==> myLabels.tex <==
\newcommand{\thmlabel}[1]{\label{thm:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\twothmref}[2]{Theorems~\ref{thm:#1} and \ref{thm:#2}}
\newcommand{\threethmref}[3]{Theorems~\ref{thm:#1}, \ref{thm:#2} and \ref{thm:#3}}

\newcommand{\lemlabel}[1]{\label{lem:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\twolemref}[2]{Lemmata~\ref{lem:#1} and \ref{lem:#2}}
\newcommand{\threelemref}[3]{Lemmata~\ref{lem:#1}, \ref{lem:#2} and \ref{lem:#3}}

\newcommand{\eqnlabel}[1]{\label{eqn:#1}}
\newcommand{\eqnref}[1]{\eqref{eqn:#1}}
\newcommand{\Eqnref}[1]{Equation~\eqref{eqn:#1}}
\newcommand{\twoEqnref}[2]{Equations~\eqref{eqn:#1} and \eqref{eqn:#2}}

\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\Figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\figsref}[1]{Figures~\ref{fig:#1}}
\newcommand{\twofigref}[2]{Figures~\ref{fig:#1} and \ref{fig:#2}}
\newcommand{\twoFigref}[2]{Figures~\ref{fig:#1} and \ref{fig:#2}}

\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\twosecref}[2]{Sections~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\threesecref}[3]{Sections~\ref{sec:#1}, \ref{sec:#2} and \ref{sec:#3}}
\newcommand{\manysecref}[2]{Sections~\ref{sec:#1}--\ref{sec:#2}}
\newcommand{\mySection}[2]{\section{#1}\seclabel{#2}}
\newcommand{\mySubSection}[2]{\subsection{#1}\seclabel{#2}}

\newcommand{\corlabel}[1]{\label{cor:#1}}
\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\twocorref}[2]{Corollaries~\ref{cor:#1} and \ref{cor:#2}}

\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\twotabref}[2]{Tables~\ref{tab:#1} and \ref{tab:#2}}

\newcommand{\proplabel}[1]{\label{prop:#1}}
\newcommand{\propref}[1]{Proposition~\ref{prop:#1}}
\newcommand{\twopropref}[2]{Propositions~\ref{prop:#1} and \ref{prop:#2}}

\newcommand{\conjlabel}[1]{\label{con:#1}}
\newcommand{\conjref}[1]{Conjecture~\ref{con:#1}}    

\newcommand{\exlabel}[1]{\label{ex:#1}}
\newcommand{\exref}[1]{Example~\ref{ex:#1}}

\newcommand{\alglabel}[1]{\label{alg:#1}}
\newcommand{\algref}[1]{Algorithm~\ref{alg:#1}}

\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}

\newcommand{\claimlabel}[1]{\label{claim:#1}}
\newcommand{\claimref}[1]{Claim~\ref{claim:#1}}
\newcommand{\twoclaimref}[2]{Claims~\ref{claim:#1} and \ref{claim:#2}}

\newcommand{\factlabel}[1]{\label{fact:#1}}
\newcommand{\factref}[1]{Fact~\ref{fact:#1}}

\newcommand{\itemlabel}[1]{\label{it:#1}}
\newcommand{\itemref}[1]{\ref{it:#1}}    
\newcommand{\itlabel}[1]{\label{it:#1}}

\newcommand{\obslabel}[1]{\label{obs:#1}}
\newcommand{\obsref}[1]{Observation~\ref{obs:#1}}
\newcommand{\twoobsref}[2]{Observations~\ref{obs:#1} and \ref{obs:#2}}

\newcommand{\openlabel}[1]{\label{open:#1}}
\newcommand{\openref}[1]{Open Problem~\ref{open:#1}}    

\newcommand{\queslabel}[1]{\label{ques:#1}}
\newcommand{\quesref}[1]{Question~\ref{ques:#1}}

\newcommand{\stepref}[1]{Step~\ref{it:#1}}    
\newcommand{\stepsref}[2]{\mbox{Steps~\ref{it:#1}--\ref{it:#2}}}


